Shape of Motion: 4D Reconstruction from a Single Video

Monocular dynamic reconstruction is a challenging and long-standing vision problem due to the highly ill-posed nature of the task. Existing approaches depend on templates, are effective only in quasi-static scenes, or fail to model 3D motion explicitly. We introduce a method for reconstructing generic dynamic scenes, featuring explicit, persistent 3D motion trajectories in the world coordinate frame, from casually captured monocular videos. We tackle the problem with two key insights: First, we exploit the low-dimensional structure of 3D motion by representing scene motion with a compact set of SE(3) motion bases. Each point's motion is expressed as a linear combination of these bases, facilitating soft decomposition of the scene into multiple rigidly-moving groups. Second, we take advantage of off-the-shelf data-driven priors such as monocular depth maps and long-range 2D tracks, and devise a method to effectively consolidate these noisy supervisory signals, resulting in a globally consistent representation of the dynamic scene. Experiments show that our method achieves state-of-the-art performance for both long-range 3D/2D motion estimation and novel view synthesis on dynamic scenes. Project Page: https://shape-of-motion.github.io/

==> define.tex <==
\newcommand{\vickie}[1]{{\color{orange}[VY: #1]}}
\newcommand{\qw}[1]{{\color{blue}[QW: #1]}}
\newcommand{\ak}[1]{{\color{red}[AK: #1]}}
\newcommand{\hangg}[1]{{\color{teal}[HG: #1]}}
\newcommand{\new}[1]{{\color{blue}}}
\newcommand{\weijia}[1]{{\color{green}[WZ: #1]}

\newcommand{\deltaavg}{<\hspace{-0.2em}\delta_{\text{avg}}}
\newcommand{\smallthreedth}{.05}
\newcommand{\largethreedth}{.10}
\newcommand{\deltathreedsmall}{\delta_{3D}^{\smallthreedth}}
\newcommand{\deltathreedlarge}{\delta_{3D}^{\largethreedth}}
\newcommand{\tf}[1]{\mathbf{#1}}
\newcommand{\Gt}{\mathbf{G}_t}
\newcommand{\world}{{}^{\textrm{w}}}
\newcommand{\cam}{{}^{\textrm{c}}}

\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\keywords}[1]{\textbf{Keywords:} #1}


\newcommand{\gmean}{\boldsymbol{\mu}}
\newcommand{\gcovariance}{\mathbf{\Sigma}}
\newcommand{\grot}{\mathbf{R}}
\newcommand{\gscale}{\mathbf{s}}
\newcommand{\gopacity}{o}
\newcommand{\gcolor}{\mathbf{c}}
\newcommand{\motionbasis}{\mathbf{T}}
\newcommand{\motioncoef}{\mathbf{w}}
\newcommand{\SETHREE}{\mb{SE}(3)}
\newcommand{\ftf}[3]{{#1}_{#3 \rightarrow #2}}
